On the intrinsic dimensionality of Covid-19 data: a global perspective

This paper aims to develop a global perspective of the complexity of the relationship between the standardised per-capita growth rate of Covid-19 cases, deaths, and the OxCGRT Covid-19 Stringency Index, a measure describing a country's stringency of lockdown policies. To achieve our goal, we use a heterogeneous intrinsic dimension estimator implemented as a Bayesian mixture model, called Hidalgo. We identify that the Covid-19 dataset may project onto two low-dimensional manifolds without significant information loss. The low dimensionality suggests strong dependency among the standardised growth rates of cases and deaths per capita and the OxCGRT Covid-19 Stringency Index for a country over 2020-2021. Given the low dimensional structure, it may be feasible to model observable Covid-19 dynamics with few parameters. Importantly, we identify spatial autocorrelation in the intrinsic dimension distribution worldwide. Moreover, we highlight that high-income countries are more likely to lie on low-dimensional manifolds, likely arising from aging populations, comorbidities, and increased per capita mortality burden from Covid-19. Finally, we temporally stratify the dataset to examine the intrinsic dimension at a more granular level throughout the Covid-19 pandemic.

==> cover_letter.tex <==


Professor X
Journal of ….

Feb-2022

Dear Professor X: 

Please, find enclosed the manuscript “On the intrinsic dimensionality of Covid-19 data: a global perspective”, that we would like to submit for publication in the Journal of ... 

[Add an intro here]

In this article, we …

We include a novel analysis of …

We believe that this article could be of interest to a broad audience and particularly to the readership of ... 

[Suggested reviewers]

\section{Author summary}
The novel coronavirus SARS-CoV-2 (Covid-19) pandemic has caused severe suffering and death worldwide. In less than two years, it has disrupted countries' economies, caused the collapse of the medical systems, and produced massive death tolls. While previous research has looked at different aspects of the transmission of the virus, little work has been done to reveal the latent dynamics of the pandemic spread across continents and countries. Global Covid-19 statistics produce high-dimensional longitudinal data, which are challenging for statistical inference and decision making. Given the complex nature of the dataset, we aim at uncovering hidden patterns monitoring its intrinsic dimension (ID), which can be seen as an index of complexity of the data. In this work, we use a recently developed Bayesian mixture model, the heterogeneous ID algorithm, Hidalgo. This model is capable of segmenting data into groups characterized by homogeneous intrinsic dimension, allowing for the presence of heterogeneous manifolds. This work identifies that the selected Covid-19 statistics lie on a low-dimensional manifold, suggesting that Covid-19 data dynamics are generated from a latent mechanism characterized by a few important variables. Furthermore, we identify a spatial relationship in the complexity of the chosen Covid-19 statistics. Lastly, we observe high-income countries tend to exhibit lower levels of underlying complexity, which we identify as arising from aging populations, the prevalence of chronic diseases, and increased per capita mortality burden from Covid-19.


Thank you for your consideration,
Yours faithfully, 


The authors:


School of Mathematical Sciences
Y Block, Floor 8, Gardens Point Campus
Queensland University of Technology
GPO Box 2434. Brisbane, QLD 4001
Australia


References

